Annealing Optimisation of Mixed ZX Phase Circuits

We present a topology-aware optimisation technique for circuits of mixed ZX phase gadgets, based on conjugation by CX gates and simulated annealing.

==> eptcsdata.tex <==
\providecommand{\firstpage}{415}
\providecommand{\publicationstatus}{S. Gogioso, M. Hoban (Eds.):\\
Quantum Physics and Logic (QPL) 2022\\
EPTCS 394, 2023, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.394.20}{10.4204/EPTCS.394.20}}
\pdfoutput=1

